Deep Learning for In-Orbit Cloud Segmentation and Classification in Hyperspectral Satellite Data

This article explores the latest Convolutional Neural Networks (CNNs) for cloud detection aboard hyperspectral satellites. The performance of the latest 1D CNN (1D-Justo-LiuNet) and two recent 2D CNNs (nnU-net and 2D-Justo-UNet-Simple) for cloud segmentation and classification is assessed. Evaluation criteria include precision and computational efficiency for in-orbit deployment. Experiments utilize NASA's EO-1 Hyperion data, with varying spectral channel numbers after Principal Component Analysis. Results indicate that 1D-Justo-LiuNet achieves the highest accuracy, outperforming 2D CNNs, while maintaining compactness with larger spectral channel sets, albeit with increased inference times. However, the performance of 1D CNN degrades with significant channel reduction. In this context, the 2D-Justo-UNet-Simple offers the best balance for in-orbit deployment, considering precision, memory, and time costs. While nnU-net is suitable for on-ground processing, deployment of lightweight 1D-Justo-LiuNet is recommended for high-precision applications. Alternatively, lightweight 2D-Justo-UNet-Simple is recommended for balanced costs between timing and precision in orbit.

==> 7-Draft_comments.tex <==



% \newpage
\clearpage

\subsubsection*{Comments}

\section*{Introduction}

MAIN AUTHOR: BUT\\

\begin{itemize}
    \item general intro ... conference is mainly focused on signal processing so that we can address the first paragraph generally \JON{ok, but establish the relation between neural networks for solving signal processing tasks (convolution, etc)} \JANO{sure}
    \item why is advantageous to process data on-board \JON{as an idea, you could mention that one of the tasks of interest is image segmentation on-board, and for this you can check Figure 2 in our article where we explain that data processing aboard the satellite can help automate the payload, make a more efficient use of the on-board memory resources, power consumption aboard the satellite, more efficient downlink, etc - article here: https://arxiv.org/pdf/2310.16210.pdf } \JANO{Here we will focus more in our use-case based on project, but in general is the same} \JJON{No problem! It makes sense, no problem. It's even interesting for us to see other use-cases.} 
    \item Why to use hyperspectral data \JON{and benefits of using hyperspectral over multispectral as well as drawbacks} \JANO{agree}
    \item \Zolo{I've put a general intro above, @jano, @daniel, please check} \Daniel{great}
    \item \Daniel{We should set a goal at the end of the intro: find the best model for cloud segmentation on-board and sensor independance potential (channel selection)}
\end{itemize}

\subsection{State of the art} \label{sota}

\begin{itemize}
    \item address Jon's work \JON{I could write this part. I could describe in a neutral way what the experiments were about and which conclusions were achieved - basically what it can be found in the abstract and the conclusion} \JANO{Yes please, try to fit to one paragraph maybe?} \JJON{Yes, I'll do so. If it's ok, when you have filled text in the intro and I can see the flow of the intro, I can add some text (if I see the flow you have in mind it will be easier for me to write)}
    \item if there will be space, put some works on the table 
    \item switch to goals/novelty of our work \JON{I know these can be harder questions, but I think we should try to address them: what's new? have we done a thorough state-of-the-art study? what does this work do that other works are not doing? why is that important?} \JANO{Yes, but usually we are fitting them more based on results :) }
\end{itemize}

\section*{Dataset}

MAIN AUTHOR: ZAITRA\\
Please describe the dataset: 
\begin{itemize}
    \item Dataset EO1 - approx. 500 tiles 254x254 
    \item source mission \JON{exactly! what is the scientific purpose of the mission}
    \item imager 
    \item bands-ranges \JON{and comment on the spectral and spatial resolutions}
    \item amount of data \JON{both in terms of images and perhaps, if you think it is suited, in terms of the number of spectral sigantures}
    \item pre-processing (radiometry, etc.) \JON{state VERY CLEARLY what level(s) you're using}
    \item cloud distribution \JON{what does cloud distribution mean in this context? detection of clouds?}
    \item tilling process 
    \item example (3 tiles in a new row) 

\end{itemize}

\section*{Machine Learning}

...\\

\begin{enumerate}
    \item ML
        \begin{enumerate}
            \item 3 networks justified by SOTA (nnUnet, 2D CUNet++, 1D Justo-Liu-Net) \JON{I can justify why 2D CUNet++ and 1D-Justo-LiuNet are being tested}
            \JANO{We will prepare this section and then we will mark where you can put your input} \JJON{Perfect, thank you!} \Daniel{I think it is 2D-Justo-UNet-Simple, which gives the best results based on Jon's paper. I've trained this model}
            \item training - begin with 100 epochs, other params based on network \JON{perhaps too soon to judge, but I must admit that when I read the number of epochs I was like: woow! 100 epochs? In the case of HYPSO we only used 2-3 epochs to avoid overfitting. Of course, it depends on the data. In any case, plan carefully how you will be selecting the training parameters and hyperparameters and if you will be doing any hyper-parameter tuning optimization.}
            \JANO{We discussed this, and we reduce to 20 epochs for the beginning, nevertheless nnUnet is by default set to 1000 epochs, so that is why we used 100 epochs. 2-3 seems to be a bit low for now, but let us see..} \JJON{I actually agree, 2 and 3 epochs sounds low, even I thought about that when I wrote our last paper. I guess the early-stopping criterium can change much depending on the training dataset.}
            \item train/val/test - 70/20/10 \JON{Here, I would need to see also absolute numbers to see if the distribution is good enough. I can propose for instance: 70/15/15 - so, basically increase by 5 percent the testing ratio. Furthermore, I would strongly recommend that you use an additional fourth set that many times is referred as the deployment set to further test the generalisation of the models. So, first you run tests on the testing set and measure metrics (agree with this), but then a deployment set is needed to evaluate more extensively the generalisation of the model. This deployment set does not need to be labeled, many authors evaluate the results subjectively in case of abscence of ground-truth (we did the same for HYPSO). I think a deployment prove further the models are reliable.}
            \JANO{I do not see a reason for 4th set from the same dataset as testing data will be excluded from the training loop. We will have commercial data for the subjective test as you mentioned} \JJON{I think that here my key point was that there should be an extensive fourth set. If we can manage to have a fourth set from a different source (commercial data) that would be even better. In our case, since we didn't have commercial data, for the fourth extensive set we just had to use the same data source :(}
            \item additional test will be made by new commercial data (100 labeled tiles of different datasets - description to Section 2?) \JON{is this part of your testing for other data sources? In this case, again the level of radiometric correction should be clearly stated :)}
            \item Scenarios:
                \begin{enumerate}
                    \item 1-band only (best by PCA) \JON{Any justification for only one band? any state of the art doing the same?}
                    \JANO{We just want to see what is happening with performance in terms of resource consumption}
                    \item all bands
                    \item selected 7-9 bands by PCA \JON{Again, why 7-9 bands?}
                    \JANO{Based on PCA, we already now results :D } \JJON{I see, I see! Perfect!}
                \end{enumerate}
            \item Metrics segmentation - IoU, Jaccard Index, Dice, Pixel ACC
            \item Metrics classification - ACC, PRE, REC, F1 \JON{Something I already noticed in the last meeting was that there was a large number of metrics. I think it is good that we are measuring various metrics, and we indeed did the same for HYPSO, but I think that for later analyzing results and concluding it will be easier to focus in a smaller set of metrics (this is a typical comment reviewers within AI may give). For instance, instead of using precision, recall, and F1-Score we can use only F1-Score which already accounts for the harmonic mean of the precision and the recall. Also, as regards IoU, Jaccard Index (etc) we should choose which ones to pick. TIP: Check which metrics have been used in the state of the art for hyperspectral segmentation. You can check which metrics we used in the supplementary material in \url{https://github.com/NTNU-SmallSat-Lab/s_l_c_segm_hyp_img/} (click on where it says Remaining material)}
            \JANO{This is intentional, for the final result-table we will use just a subset of metrics that will have the best description meaning for discussion} \JJON{Exactly, completely agree! For me it was very useful to have my own excel document where I was writing down the metrics, and then I chose the ones that were relevant for the discussion and previously used in sota}
            \item Metrics regarding the FPGA - Memory size, inference time, FLOPS, number of params \JON{I agree these parameters are important but we should reduce it to compress the scope of the paper...}
            \JANO{Sure, same as previous comment}
        \end{enumerate}



    \item Experiments flow
    \begin{enumerate}
        \item PCA
        \item 7 runs - 7 models \JON{so 3 possible input channels (all channels, only 1, only 7-9 channels) and 3 models}
        \JANO{Since 1D will be run only with all bands there will be 7 runs 3 per 2D network and one per 1D}
        \item select the best model concerning FPGA possibilities \JON{at the moment, I have doubts about if it is convenient to have this conclusion in this paper as I think further analysis might be needed to conclude with strong basis which model is suited for FPGA}
        \JANO{This will not be final/general conclusion, just pilot/preliminary one since we are heading for conference. For final decision we need to run models on FPGA, what is out of the scope} \JJON{Perfect, I agree, and as you say it is something preliminary.}
        \item evaluate on the commercial dataset \JON{is this from another sensor?} \JJON{All clear now!}
        \JANO{Yes.}
    \end{enumerate}
\end{enumerate}

\section*{Results}
MAIN AUTHOR: BUT\\

\section*{Discussion}
MAIN AUTHOR: BUT+ZAITRA+NTNU\\



